Study of the $D^0 p$ amplitude in $\Lambda_b^0\to D^0 p \pi^-$ decays

An amplitude analysis of the decay $\Lambda_b^0\to D^0 p \pi^-$ is performed in the part of the phase space containing resonances in the $D^0 p$ channel. The study is based on a data sample corresponding to an integrated luminosity of 3.0 fb$^{-1}$ of $pp$ collisions recorded by the LHCb experiment. The spectrum of excited $\Lambda_c^+$ states that decay into $D^0 p$ is studied. The masses, widths and quantum numbers of the $\Lambda_c(2880)^+$ and $\Lambda_c(2940)^+$ resonances are measured. The constraints on the spin and parity for the $\Lambda_c(2940)^+$ state are obtained for the first time. A near-threshold enhancement in the $D^0 p$ amplitude is investigated and found to be consistent with a new resonance, denoted the $\Lambda_c(2860)^+$, of spin $3/2$ and positive parity.

==> LHCb_Authorship_flat_arXiv_15-Nov-2016.tex <==
LHCb collaboration: 
R. Aaij,
B. Adeva,
M. Adinolfi,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
S. Ali,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
S. Amerio,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
R.B. Appleby,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
E. Aslanides,
G. Auriemma,
M. Baalouch,
I. Babuschkin,
S. Bachmann,
J.J. Back,
A. Badalov,
C. Baesso,
S. Baker,
V. Balagura,
W. Baldini,
R.J. Barlow,
C. Barschel,
S. Barsuk,
W. Barter,
F. Baryshnikov,
M. Baszczyk,
V. Batozskaya,
B. Batsukh,
V. Battista,
A. Bay,
L. Beaucourt,
J. Beddow,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
A. Berezhnoy,
R. Bernet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.-O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bifani,
P. Billoir,
T. Bird,
A. Birnkraut,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J. Blouw,
S. Blusk,
V. Bocci,
T. Boettcher,
A. Bondar,
N. Bondar,
W. Bonivento,
I. Bordyuzhin,
A. Borgheresi,
S. Borghi,
M. Borisyak,
M. Borsato,
F. Bossu,
M. Boubdir,
T.J.V. Bowcock,
E. Bowen,
C. Bozzi,
S. Braun,
M. Britsch,
T. Britton,
J. Brodzicka,
E. Buchanan,
C. Burr,
A. Bursche,
J. Buytaert,
S. Cadeddu,
R. Calabrese,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carson,
K. Carvalho Akiba,
G. Casse,
L. Cassina,
L. Castillo Garcia,
M. Cattaneo,
G. Cavallero,
R. Cenci,
D. Chamont,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
S. Chen,
S.-F. Cheung,
V. Chobanova,
M. Chrzaszcz,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J. Cogan,
E. Cogneras,
V. Cogoni,
L. Cojocariu,
G. Collazuol,
P. Collins,
A. Comerma-Montells,
A. Contu,
A. Cook,
G. Coombs,
S. Coquereau,
G. Corti,
M. Corvo,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
S. Cunliffe,
R. Currie,
C. D'Ambrosio,
F. Da Cunha Marinho,
E. Dall'Occo,
J. Dalseno,
P.N.Y. David,
A. Davis,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.T. Dean,
D. Decamp,
M. Deckenhoff,
L. Del Buono,
M. Demmer,
A. Dendek,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Canto,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
K. Dungs,
P. Durante,
R. Dzhelyadin,
A. Dziurda,
A. Dzyuba,
N. D{\'e}l{\'e}age,
S. Easo,
M. Ebert,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
S. Ely,
S. Esen,
H.M. Evans,
T. Evans,
A. Falabella,
N. Farley,
S. Farry,
R. Fay,
D. Fazzini,
D. Ferguson,
A. Fernandez Prieto,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiore,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
K. Fohl,
M. Fontana,
F. Fontanelli,
D.C. Forshaw,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
W. Funk,
E. Furfaro,
C. F{\"a}rber,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
P.J. Garsed,
D. Gascon,
C. Gaspar,
L. Gavardi,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Ph. Ghez,
S. Gian{\`\i},
V. Gibson,
O.G. Girard,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
P. Griffith,
L. Grillo,
B.R. Gruberg Cazon,
O. Gr{\"u}nberg,
E. Gushchin,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
B. Hamilton,
X. Han,
S. Hansmann-Menzemer,
N. Harnew,
S.T. Harnew,
J. Harrison,
M. Hatch,
J. He,
T. Head,
A. Heister,
K. Hennessy,
P. Henrard,
L. Henry,
E. van Herwijnen,
M. He{\ss},
A. Hicheur,
D. Hill,
C. Hombach,
H. Hopchev,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
P. Ilten,
R. Jacobsson,
A. Jaeger,
J. Jalocha,
E. Jans,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
M. Kecke,
M. Kelsey,
M. Kenzie,
T. Ketel,
E. Khairullin,
B. Khanji,
C. Khurewathanakul,
T. Kirn,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
M. Kolpin,
I. Komarov,
R.F. Koopman,
P. Koppenburg,
A. Kosmyntseva,
A. Kozachuk,
M. Kozeiha,
L. Kravchuk,
K. Kreplin,
M. Kreps,
P. Krokovny,
F. Kruse,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
A.K. Kuonen,
K. Kurek,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
J. van Leerdam,
A. Leflat,
J. Lefran{\c{c}}ois,
R. Lef{\`e}vre,
F. Lemaitre,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
B. Leverington,
T. Li,
Y. Li,
T. Likhomanenko,
R. Lindner,
C. Linn,
F. Lionetto,
X. Liu,
D. Loh,
I. Longstaff,
J.H. Lopes,
D. Lucchesi,
M. Lucio Martinez,
H. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
O. Maev,
K. Maguire,
S. Malde,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
P. Manning,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
G. Martellotti,
M. Martin,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
D. Martins Tostes,
L.M. Massacrier,
A. Massafferri,
R. Matev,
A. Mathad,
Z. Mathe,
C. Matteuzzi,
A. Mauri,
E. Maurice,
B. Maurin,
A. Mazurov,
M. McCann,
A. McNab,
R. McNulty,
B. Meadows,
F. Meier,
M. Meissner,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
M.-N. Minard,
D.S. Mitzel,
A. Mogini,
J. Molina Rodriguez,
I.A. Monroy,
S. Monteil,
M. Morandin,
P. Morawski,
A. Mord{\`a},
M.J. Morello,
O. Morgunova,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mulder,
M. Mussini,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
M. Neuner,
T.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
T. Nikodem,
A. Nogay,
A. Novoselov,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
J.M. Otalora Goicochea,
A. Otto,
P. Owen,
A. Oyanguren,
P.R. Pais,
A. Palano,
M. Palutan,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
G.D. Patel,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
M. Petruzzo,
E. Picatoste Olloqui,
B. Pietrzyk,
M. Pikies,
D. Pinci,
A. Pistone,
A. Piucci,
V. Placinta,
S. Playfer,
M. Plo Casasus,
T. Poikela,
F. Polci,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
A. Popov,
D. Popov,
B. Popovici,
S. Poslavskii,
C. Potterat,
E. Price,
J.D. Price,
J. Prisciandaro,
A. Pritchard,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
G. Punzi,
W. Qian,
R. Quagliani,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
I. Raniuk,
F. Ratnikov,
G. Raven,
F. Redi,
S. Reichert,
A.C. dos Reis,
C. Remon Alepuz,
V. Renaudin,
S. Ricciardi,
S. Richards,
M. Rihl,
K. Rinnert,
V. Rives Molina,
P. Robbe,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
P. Rodriguez Perez,
A. Rogozhnikov,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
J.W. Ronayne,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
P. Ruiz Valls,
J.J. Saborido Silva,
E. Sadykhov,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
A. Sarti,
C. Satriano,
A. Satta,
D.M. Saunders,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schlupp,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
K. Schubert,
M. Schubiger,
M.-H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
P. Seyfert,
M. Shapkin,
I. Shapoval,
Y. Shcheglov,
T. Shears,
L. Shekhtman,
V. Shevchenko,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
M. Sirendi,
N. Skidmore,
T. Skwarnicki,
E. Smith,
I.T. Smith,
J. Smith,
M. Smith,
H. Snoek,
l. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
P. Spradlin,
S. Sridharan,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
H. Stevens,
S. Stevenson,
S. Stoica,
S. Stone,
B. Storaci,
S. Stracka,
M. Straticiuc,
U. Straumann,
L. Sun,
W. Sutcliffe,
K. Swientek,
V. Syropoulos,
M. Szczekowski,
T. Szumlak,
S. T'Jampens,
A. Tayduganov,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
S. Topp-Joergensen,
F. Toriello,
E. Tournefier,
S. Tourneur,
K. Trabelsi,
M. Traill,
M.T. Tran,
M. Tresch,
A. Trisovic,
A. Tsaregorodtsev,
P. Tsopelas,
A. Tully,
N. Tuning,
A. Ukleja,
A. Ustyuzhanin,
U. Uwer,
C. Vacca,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
G. Veneziano,
A. Venkateswaran,
M. Vernet,
M. Vesterinen,
J.V. Viana Barbosa,
B. Viaud,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
M. Vitti,
V. Volkov,
A. Vollhardt,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
C. Vo{\ss},
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
C. Wallace,
R. Wallace,
J. Walsh,
J. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
M. Whitehead,
J. Wicht,
G. Wilkinson,
M. Wilkinson,
M. Williams,
M.P. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
J. Wimberley,
J. Wishahi,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wraight,
K. Wyllie,
Y. Xie,
Z. Xing,
Z. Xu,
Z. Yang,
Y. Yao,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
L. Zhang,
Y. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhu,
V. Zhukov,
S. Zucchelli

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

